One-Shot Imitation under Mismatched Execution

Human demonstrations as prompts are a powerful way to program robots to do long-horizon manipulation tasks. However, translating these demonstrations into robot-executable actions presents significant challenges due to execution mismatches in movement styles and physical capabilities. Existing methods for human-robot translation either depend on paired data, which is infeasible to scale, or rely heavily on frame-level visual similarities that often break down in practice. To address these challenges, we propose RHyME, a novel framework that automatically pairs human and robot trajectories using sequence-level optimal transport cost functions. Given long-horizon robot demonstrations, RHyME synthesizes semantically equivalent human videos by retrieving and composing short-horizon human clips. This approach facilitates effective policy training without the need for paired data. RHyME successfully imitates a range of cross-embodiment demonstrators, both in simulation and with a real human hand, achieving over 50% increase in task success compared to previous methods. We release our code and datasets at https://portal-cornell.github.io/rhyme/.

==> paper/algorithms/algos.tex <==

\noindent % Ensures no indentation which might mess with alignment

\begin{minipage}[t]{0.50\textwidth}
\vspace{-7mm}
    \input{paper/algorithms/rhyme_algo}
\end{minipage}
\hfill % This will create space between the two minipages
\begin{minipage}[t]{0.48\textwidth}
\vspace{-7mm}
    \input{paper/algorithms/retrieval_algo}
\end{minipage}


==> paper/algorithms/hyper.tex <==


% \setlength{\tabcolsep}{0.1cm}
{
\begin{tabular}{ll}
\toprule

\textsc{Imagine-Demo} Hyperparam. $\downarrow$ & Value\\
\midrule
OT similarity temperature             & 0.05 \\
TCC similarity temperature            & 0.1 \\
\midrule

Policy $\pi$ Hyperparam.~\cite{chi2023diffusion}$\downarrow$ & Value \\
\midrule
Observation Horizon            & 2   \\
Action Horizon                 & 2    \\
Action Pred. Horizon            & 16   \\
State - Vision Feature Dim.        & 64     \\
State - Proprio. Feature Dim.           & 9 \\
Action Dim.           & 9 \\
Batch Size                 & 128    \\
Training iteration         & 200   \\
Learning rate              & 1e-4  \\
Weight decay              & 1e-6  \\
Optimizer                 & ADAM  \\ 
\bottomrule
\end{tabular}%
}
\label{tab:sim_hyper}


==> paper/algorithms/hyper_vid.tex <==


% \setlength{\tabcolsep}{0.1cm}
{
\begin{tabular}{ll}
\toprule
Video Encoder $\phi$ Hyperparam.~\cite{xu2023xskill} $\downarrow$ & Value\\
\midrule
Video Clip length   $l$       & 8     \\
Sampling Frames  $T$           & 100   \\
Sinkhorn iterations        & 3     \\
Sinkhorn epsilon           & 0.03  \\
Prototype loss coef        & 0.5   \\
Prototype loss temperature & 0.1   \\
TCN loss coef & 1     \\
TCN positive window  $w_p$      & 4     \\
TCN negative window  $w_n$      & 12    \\
TCN negative samples       & 16    \\
TCN temperature   $\tau_{\text{tcn}}$         & 0.1   \\
Batch Size                 & 28    \\
Training iteration         & 100   \\
Learning rate              & 1e-4  \\
Optimizer                 & ADAM  \\ 
\bottomrule
\end{tabular}%
}
\label{tab:sim_hyper}


==> paper/algorithms/planning_bcz.tex <==
\begin{algorithm}[t!]
  \caption{BC-Z}
  \begin{algorithmic}[1]
    \State \textbf{Input:} Robot Trajectories $\xi_R = \{\xi_R^0, \xi_R^1, \xi_R^2, \dots \xi_R^N\}$, Corresponding Human Trajectories = $\xi_H = \{\xi_H^0, \xi_H^1, \xi_H^2, \dots \xi_H^N\}$, Aligned Feature Space $\phi$, Expert Human Demo $\xi_H^* = \{ s_0^H, s_1^H, \dots, s_T^H \}$
    \State \textbf{Training Pipeline}
    \State Dataset $D = \{ \}$
    \For{$\xi_R^i = \{ (s_0^R,a_0^R), (s_1^R,a_1^R), \dots, (s_T^R,a_T^R) \} \in \xi_R, \xi_H^i \in \xi_H$}
        \For{$s_t^R \in \xi_R$}
            \State $s_{t*}^H = \argmin_{s_{t'}^H} d(\phi(s_t^R), \phi(s_t'^H))$ \Comment{\textbf{Find nearest neighbor in human video}}
            \State Sample $\triangle t$ looking ahead from timestep $t*$ \Comment{Lookahead subgoal from current}
            \State Add tuple $(s_t^R, a_t^R, g_t^H = s_{t*+\triangle t}^H)$ to $D$
        \EndFor
    \EndFor

    \State Train model $\pi(a_t^R | s_t^R, g_t^H)$ using Dataset $D$


    \State \textbf{Inference Pipeline}
    \State At Current Robot State $s_t^R$,
    \State Let $s_{t*}^H = \argmin_{s_{t'}^H} d(\phi(s_t^R), \phi(s_t'^H))$ \Comment{Find nearest neighbor in human video}
    \State $g_{t}^H = s_{t*+\triangle t}^H$
    \Comment{Lookahead from that frame}
    \State $a_t^R = \pi(. | s_t^R, g_t^H)$ \Comment{Zero shot policy to a human subgoal frame}
    
  \end{algorithmic}
\end{algorithm}

==> paper/algorithms/planning_preference.tex <==
\begin{algorithm}[t!]
  \caption{Few-Shot Transfer (OURS)}
  \begin{algorithmic}[1]
    \State \textbf{Input:} Robot Trajectories $\xi_R = \{\xi_R^0, \xi_R^1, \xi_R^2, \dots \xi_R^N\}$, Unaligned Human Trajectories = $\xi_H = \{\xi_H^0, \xi_H^1, \xi_H^2, \dots \xi_H^N\}$, Aligned Feature Space $\phi$, Expert Human Demo $\xi_H^* = \{ s_0^H, s_1^H, \dots, s_T^H \}$
    \State \textbf{Training Pipeline}
    \State Dataset $D = \{ \}$
    \For{$\xi_R^i = \{ (s_0^R,a_0^R), (s_1^R,a_1^R), \dots, (s_T^R,a_T^R) \} \in \xi_R$}
        \State $\xi_H^j = \argmin_{\xi_H^j} d(\phi(\xi_R^i), \phi(\xi_H^j))$ \Comment{\textbf{Find nearest human video to current human video}}
        \For{$s_t^R \in \xi_R$}
            \State $s_{t*}^H = \argmin_{s_{t'}^H} d(\phi(s_t^R), \phi(s_t'^H))$ \Comment{\textbf{Find nearest neighbor in human video}}
            \State Sample $\triangle t$ looking ahead from timestep $t*$ \Comment{Lookahead subgoal from current}
            \State Add tuple $(s_t^R, a_t^R, g_t^H = s_{t*+\triangle t}^H)$ to $D$
        \EndFor
    \EndFor

    \State Train model $\pi(a_t^R | s_t^R, g_t^H)$ using Dataset $D$


    \State \textbf{Inference Pipeline}
    \State At Current Robot State $s_t^R$,
    \State Let $s_{t*}^H = \argmin_{s_{t'}^H} d(\phi(s_t^R), \phi(s_t'^H))$ \Comment{Find nearest neighbor in human video}
    \State $g_{t}^H = s_{t*+\triangle t}^H$
    \Comment{Lookahead from that frame}
    \State $a_t^R = \pi(. | s_t^R, g_t^H)$ \Comment{Zero shot policy to a human subgoal frame}
    
  \end{algorithmic}
\end{algorithm}

==> paper/algorithms/planning_with_subgoals.tex <==
\begin{algorithm}[t!]
  \caption{Subgoal Planning guided by Human Trajectory}
  \begin{algorithmic}[1]
    \State \textbf{Input:} Start State $s_0$, Goal State $s_g$, Subgoal Predictor $p(. |s, s_g)$, Human Trajectory $\xi_H = \{ s_0^H, s_1^H, \dots, s_K^H \}$
    \State \textbf{Output:} Sequence of Subgoals $\xi_R = \{ s_0^R, s_1^R, \dots, s_T^R \}$
    
    \State $\mathcal{T} \leftarrow \{S_0\}$ \algorithmiccomment{Initialize tree with Start State as root}
    
    \While{\textsc{Goal-Not-Reached}}
        \State Initialize a priority list $L$
        \For{$s_R \in \mathcal{T}$}
            \State $s_{t}^H \leftarrow$ \textsc{ClosestHumanState}$(s_R, \xi_H)$
            \If{$||s_{t}^H-s_R|| < \epsilon$}
                \State $L.append(s_R, t)$
            \EndIf
        \EndFor

        \State $s_R \leftarrow $ Select-Best$(L)$ \Comment{Select best node to expand from $L$ \\ \hfill with priority to states with higher $t$ values}

        \If{ReachedGoal$(s_R)$}
            \State ${\xi_R} \leftarrow BacktrackPlan(s_R)$ \Comment{Construct the plan by backtracking}
        \EndIf
        \State Generate $M$ plans of $H$ depth using $p(. |s_R, s_g)$ \Comment{Can optimize to reach human states}
        \State Add generated nodes into $\mathcal{T}$
    \EndWhile
    
    
    
    \State \textbf{return} ${\xi_R}$ \Comment{Return the constructed plan}
  \end{algorithmic}
\end{algorithm}


==> paper/algorithms/planning_xskills.tex <==
\begin{algorithm}[t!]
  \caption{XSKills - Zero Shot Transfer}
  \begin{algorithmic}[1]
    \State \textbf{Input:} $\xi_R = \{\xi_R^0, \xi_R^1, \xi_R^2, \dots \xi_R^N\}$, Aligned Feature Space $\phi$, Expert Human Demo $\xi_H^* = \{ s_0^H, s_1^H, \dots, s_T^H \}$
    \State \textbf{Training Pipeline}
    \State Dataset $D = \{ \}$
    \For{$\xi_R^i = \{ (s_0^R,a_0^R), (s_1^R,a_1^R), \dots, (s_T^R,a_T^R) \} \in \xi_R$}
        \State Sample $\triangle t$ looking ahead from timestep $t$ \Comment{Lookahead subgoal from current}
        \State Add tuple $(s_t^R, a_t^R, g_t^R = s_{t+\triangle t}^R)$ to $D$
    \EndFor

    \State Train model $\pi(a_t^R | s_t^R, g_t^R)$ using Dataset $D$


    \State \textbf{Inference Pipeline}
    \State At Current Robot State $s_t^R$,
    \State $s_{t*}^H = \argmin_{s_{t'}^H} d(\phi(s_t^R), \phi(s_t'^H))$ \Comment{Find nearest neighbor in human video}
    \State $g_{t}^H = s_{t*+\triangle t}^H$
    \Comment{Lookahead from that frame}
    \State $a_t^R = \pi(. | s_t^R, g_t^H)$ \Comment{Zero shot policy to a human subgoal frame}
    
  \end{algorithmic}
\end{algorithm}


==> paper/figures/approach_fig.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth, height=5cm]{example-image-a}
%     \vspace{-5mm}
%     \captionsetup{width=\textwidth}
%     \caption{\textbf{Overview of Approach.}}  
%     \label{fig:approach}
% \end{figure}

==> paper/figures/datasets.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{images/figure_dataset.png}
%     \vspace{-5mm}
%     \captionsetup{width=\textwidth}
%     \caption{\textbf{Visualizing Cross-Embodiment Datasets.} \textsc{Sphere} replaces the robot's gripper with the rendering of a sphere. \textsc{X-Sphere} moves objects differently; here lifting the kettle instead of dragging it like the robot. Additionally, the \textsc{2X-Sphere} dataset demonstrates two skills simultaneously.}  
%     \label{fig:datasets}
% \end{figure}

==> paper/related_work/cross_irl.tex <==
\subsection{Cross-Embodiment IRL}
\subsubsection{Learning Generalizable Robotic Reward Functions from "In-The-Wild" Human Videos \cite{chen2021learning}}

\subsubsection{XIRL: Cross-embodiment Inverse Reinforcement Learning \cite{zakka2022xirl}}
Goal: Enable agents to \textbf{imitate video demonstrations of experts of different embodiments} with an \textbf{embodiment-invariant reward} formulation trained with temporal cycle-consistency. 

Data: $n$ agents each with $K$ demonstrations of them completing the task. This data \textbf{only has observation data}, and not actions taken by the agents. 

Representation Learning: Use temporal cycle-consistency (TCC) to learn task-specific representations in a self-supervised way. TCC representations can predict frame-level task progress without any human annotations - it \textbf{encodes task progress in the latent space} by comparing frames of one agent performing the task with another and searching for temporal similarities in how both execute the task. Image encoder $\phi$ returns embedding vector $\phi(I)$ for an image $I$ so a random video sampled turns into a sequence of embeddings $V_i = \{\phi(v_i^1),...\}$ which is the length of the video (in num frames). From the minibatch of video sequences of the same task, compute TCC loss. Procedure: Sample frame $t$ from $V_i$, compute latent soft-nearest neighbor of that frame in $V_j$, then cycle-back by computing soft-nearest neighbor of that frame within $V_i$. The loss is the L2 distance between the original frame $t$ and the frame retrieved from cycling back. 

Reward Function: The goal embedding $g$ is the mean embedding of the last frame of all demonstration videos: $g = \sum_{i=1}^{N} \phi(v_i^{L_i})/N$ where $L_i$ is length of video. Reward $r(s) \propto -\lVert \phi(s) - g \rVert$ where $\phi(s)$ is state embedding at current timestep.

\subsubsection{What Matters to You? Towards Visual Representation Alignment for Robot Learning \cite{tian2023matters}}
Goal: Leverage human feedback to align robot visual representations with the end-user and disentangle what matters for a task.

Problem Setup:
\begin{itemize}
    \item Human Policy: Human knows desired reward $r^*$, and has approx. optimal policy mapping observations to actions. Humans also have representation model relevant to task attributes $\phi_H : O \rightarrow \varphi_H$ mapping observations to the human's latent space. 
    \item Robot Policy: $\pi_R^* = \text{arg max}_{\pi_R} E_{o \sim p(o|\pi_R)}[\sum_{t=0}^{\infty} \gamma^t \cdot r(\phi_R (o^t))]$ where robot's rewrad relies on visual representation $\phi_R$ mapping observations to lower-dim. latent space $\varphi_R$.
\end{itemize}

Triplet-Based Representation Space: For distance metric $d$, let $d(\phi(\textbf{o}^i), \phi(\textbf{o}^j))$ be distance between embedding trajectories. $S_{\phi} = \{(\textbf{o}^i, \textbf{o}^j, \textbf{o}^k) : d(\phi(\textbf{o}^i), \phi(\textbf{o}^j)) < d(\phi(\textbf{o}^i), \phi(\textbf{o}^k)), \textbf{o}^{i,j,k}\}$. For all triples of videos the agent can see, it can determine which videos are more similar using embedding space: $S_{\phi}$ contains all the similarity triplets.

Visual Representation Alignment Problem: With loss function $l$ to penalize divergence between two representation spaces, we get $\text{min}_{\phi_R} l(S_{\phi_R}, S_{\phi_H})$

Approximate the problem by obtaining a subset of triplet queries from the human, which can be used to implicity learn $\phi_H$. They seem to just do this via MLE? 

For video $o$ and representation $\phi$, induced empirical embedding distribution $\rho = \frac{1}{T}\sum_{t=0}^T \delta_{\phi(o^t)}$ where $\delta_{\phi(o^t)}$ Dirac distribution centered on the embedding. Optimal transport finds $\mu^* \in R^{T \times T}$ to transport one embedding distribution to another with minimal cost. 

Seek to match embedded observation occupancy measure induced by robot policy and that of a human's preferred video demonstration. Reward is negatively proportional to the cost? between the robot's observations and the demonstration's observations times their optimal coupling between the distributions induced by the robot and expert. 

\subsubsection{Graph Inverse Reinforcement Learning from Diverse Videos \cite{kumar2023graph}} 

==> paper/related_work/visual_rep.tex <==
\subsection{Visual Representation Alignment}
\subsubsection{Temporal Cyclic Consistency}

Intend to maximize number of points that can be mapped one-to-one by two sequences by using minimum distance in learned embedding space. Image encoder $\phi (s_i ; \theta)$ encodes two sequences of length $N$ ($u_i, ...$) and $M$ ($v_j, ...$).

Cycle-consistency: For $u_i \in U$, compute NN $v_j = \text{arg min}_{v \in V} \lVert u_i - v \rVert$ --> $u_k = \text{arg min}_{u \in U} \lVert v_j - u \rVert$. Want to maximize number of cycle-consistent points, i.e. $u_i = u_k$.

Cycle-back: Soft NN computed by taking softmax over l2 distances between each frame and using the distribution as weights to sum over frames. $\alpha_j = \frac{e^{-{\lVert u_i - v_j \rVert}^2}}{\text{normalizing factor}}$, $v' = \sum_j^M \alpha_j v_j$. From $v'$ compute probability associated with cycling back to frame $i$ and compute the soft NN back in $U$. Minimize MSE between the original and cycled back frame.

\textbf{TCC in XIRL}: They learn task-specific representations, which requires several videos from multiple embodiments per task. However, they run experiments by collecting 1000 trajectories per agent.

\subsubsection{Visual Features by Contrasting Cluster Assignments}

Compute a code (i.e. cluster assignments) from an augmented version of an image and predict the code from other augmented version of the same image. 

Features $z_t$ and $z_s$ $\rightarrow$ codes $q_t$ and $q_s$ computed by matching features to set of $K$ learnable prototype vectors in matrix $C$. $L(z_t, z_s) = l(z_t, q_s) + l(z_s, q_t)$.

Loss $l(z, q)$ is cross entropy between the code $q$ and the $K$ term distribution induced by projecting $z$ onto the $K$ prototype vectors. 

Compute codes using $C$ such that all examples in a batch are equally partitioned by prototypes (prevents trivial solution of same code for all). 

$\text{max}_Q Tr(Q^T C^T Z) + \epsilon H(Q)$, first term is to make sure the code matches the projections of the features onto the prototypes and second is entropy regularization to make sure $Q$ is a smooth mapping. $Q$ restricted to transportation polytope which makes sure each prototype is selected at least $B/K$ times in a batch. $Q*$ from optimal transport solution. 


\textbf{SwAV in XSkill}: Temporal encoder produces features from augmented images which are mapped onto $K$ learnable skill prototypes. Softmax to get probabilities $p$ over skills being executed in clip, and target distribution $q$ is generated by online Sinkhorn clustering on the projections. 

XSkill makes batches of data from same embodiment and solves entropy-regularized clustering problem which forces the data from the same embodiment to occupy the entire representation space, so clustering leads to grouping representations based on effect of skills. 

XSkill uses time contrastive loss so skill prototype probabilities are similar for temporally close video clips with InfoNCE loss. 

XSkill also uses a skill alignment transformer $\phi (z_t | o_t, \Tilde{z})$ to determine the latent skill $z_t$ to be used in the skill-conditioned policy based on the robot current observation and the entire video demonstration. Trained by sampling random features from a robot video and minimizing MSE between that feature and the prediction from using the current state and full trajectory.

\subsubsection{Preference-based Visual Alignment}

For representation encoder $\phi$, define triplet-based representation space $S_{\phi} = \{\text{demonstration triplets in order of similarity}\}$ so that the distance between the first and second demonstrations is less than that of the first and third. Approximate human's representation $\phi_H$ from a subset of $S_{\phi_H}$, to get an ordering of reward preferences.

MLE for $\Tilde{\phi_H} = \text{max}_{\phi_H} \sum_{(o^i, o^j, o^k) \in S_{\phi_H}} P(o^i \succ o^j \succ o^k | \phi_H)$

Matching embedded observation occupancy measure from robot policy $\pi_R$ to that of human's preferred video demonstration $o_+$ gives reward function: 

$r(o_r^t;\phi_R) = -\sum_{t'=1}^T c(\phi_R(o_R^t), \phi_R(o_+^{t'})*\mu_{t,t'}^*$

where $\mu^*$ is optimal coupling between induced distributions. Want the cost to be low when comparing current robot observation with the human demonstration. I assuming the coupling term will have high probability if the robot frame at $t$ and human frame at $t'$ are similar, in which case the resulting observations should also be similar? 

Induced empirical embedding distributions are defined to be average over T Dirac distributions centered on each $\phi_R(o^t)$


==> paper/tables/segment_ablation.tex <==
\begin{table}[h]
\centering

% \vspace{3pt}
% \renewcoand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|cccc|c}
\toprule
& Video Splits $K'$ $\xrightarrow{}$  & \multicolumn{4}{c|}{\textsc{RHyME-OT}} \\  
\cmidrule{3-3} \cmidrule{4-6} \cmidrule{7-7}
& Metric $\downarrow$ & $K'=1$ & $K'=2$ & $K'=3$ & $K'=4$ \\ 
\midrule
\parbox[t]{2pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{\textsc{Hard}}}}}
   & Task Recall & 49\% ($\pm$ 2.9) & 53\% ($\pm$ 3.6) & 58\% ($\pm$ 4.5) & 53\% ($\pm$ 2.6)\\
 & Task Imprecision & 28\% ($\pm$ 4.2) & 21\% ($\pm$ 3.7) & $\tbcolorg$ 12\% ($\pm$ 3.8) & 14\% ($\pm$ 3.7) \\

% \midrule
% \hline
\bottomrule

\end{tabular}
}

\vspace{3pt}
\caption{\small{We report Task Recall and Task Imprecision rates when varying the number of short horizon segments $K'$ we divide each long-horizon robot demonstration into to perform retrievals with RHyME-OT on the Sphere-Hard dataset}}.

\label{tab:seg_length}
\vspace{-5mm}
\end{table}

==> paper/tables/success_rates.tex <==
\begin{table}[h]
\centering

% \vspace{3pt}
% \renewcoand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|ccc|cc}
\toprule
& Model $\xrightarrow{}$  & \multicolumn{1}{c}{\textsc{Baseline}} & \multicolumn{2}{c|}{\textsc{Ours}} & \multicolumn{1}{c}{\textsc{Gold Standard}}\\  
\cmidrule{3-3} \cmidrule{4-5} \cmidrule{6-6}
& Metric $\downarrow$ & \textsc{XSkill} & \textsc{RHyME-TCC} & \textsc{RHyME-OT} & \textsc{OraclePairing}\\ 
\midrule
\parbox[t]{2pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{\textsc{Easy}}}}}
 & Task Recall & 82\% ($\pm$ 3.5) & 75\% ($\pm$ 1.7) &  96\% ($\pm$ 1.3) & 92\% ($\pm$ 2.7)\\
 & Task Imprecision & 5\% ($\pm$ 1.7) & 5\% ($\pm$ 1.7) &  5\% ($\pm$ 1.0) & 7\% ($\pm$ 2.3) \\
\midrule
\parbox[t]{2pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{\textsc{Med.}}}}}
  & Task Recall & 40\% ($\pm$ 2.7) & 57\% ($\pm$ 4.2) &  72\% ($\pm$ 5.8) & 92\% ($\pm$ 2.9)\\
 & Task Imprecision & 2\% ($\pm$ 1.1) & 51\% ($\pm$ 3.4) &  4\% ($\pm$ 1.9) & 0\% ($\pm$ .00) \\
\midrule
\parbox[t]{2pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{\textsc{Hard}}}}}
   & Task Recall & 1\% ($\pm$ 1.2) & 34\% ($\pm$ 4.2) &  53\% ($\pm$ 5.5) & 92\% ($\pm$ 2.2)\\
 & Task Imprecision & 53\% ($\pm$ 5.2) & 65\% ($\pm$ 4.5) &  28\% ($\pm$ 5.1) & 1\% ($\pm$ 1.1) \\

% \midrule
% \hline
\bottomrule

\end{tabular}
}

\vspace{3pt}
\caption{\small{We report exact metrics and standard errors for the bar plots in Fig~\ref{fig:dataset_barplot}}.}

\label{tab:success_rates}
\vspace{-5mm}
\end{table}

==> tables/table1.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{ccccccccccc}
\toprule
% & Models $\xrightarrow{}$  & \multicolumn{2}{c}{\textsc{Baselines}} && \multicolumn{6}{c}{\textsc{Learning-Based}}\\  \cmidrule{3-4} \cmidrule{6-11}
& Metrics (mm) $\downarrow$  & {\textsc{Only PreTrain}} & {\textsc{Only FineTune}} & {\textsc{Marginal}} &{\textsc{Marginal-AllHist} \cite{Wang2021MultiPerson3M}} & {\textsc{InteRACT}}\\   
% & & ADE & FDE && ADE & FDE  && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE\\
\midrule
\parbox[t]{2pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{ReactStir}}}}}
&All Joints FDE &97.7 (\pm 1.7) &68.5 (\pm 1.2) &59.5 (\pm 1.0) &61.0 (\pm 1.0) &\tbcolorg 53.7 (\pm 0.8) \\
&Hands/Wrists FDE &139.2 (\pm 2.4) &95.0 (\pm 1.6) &82.4 (\pm 1.3) &84.5 (\pm 1.3) &\tbcolorg 72.9 (\pm 1.1) \\
&T-All Joints FDE &95.9 (\pm 4.4) &66.5 (\pm 2.9) &60.4 (\pm 2.5) &61.5 (\pm 2.6) &\tbcolorg 54.4 (\pm 2.4) \\
&T-Hands/Wrists FDE &131.4 (\pm 6.1) &91.6 (\pm 4.0) &83.9 (\pm 3.5) &83.8 (\pm 3.6) &\tbcolorg 72.3 (\pm 3.3) \\
\midrule
\parbox[t]{2}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{Handover}}}}}
&All Joints FDE &89.4 (\pm 1.3) &68.3 (\pm 1.1) &62.0 (\pm 1.0) &62.0 (\pm 1.0) &\tbcolorg 57.5 (\pm 0.9) \\
&Hands/Wrists FDE &128.6 (\pm 2.0) &95.5 (\pm 1.5) &86.7 (\pm 1.4) &86.3 (\pm 1.4) &\tbcolorg 79.5 (\pm 1.3) \\
&T-All Joints FDE &124.7 (\pm 3.9) &92.4 (\pm 4.4) &86.3 (\pm 4.4) &86.0 (\pm 4.4) &\tbcolorg 79.7 (\pm 4.4) \\
&T-Hands/Wrists FDE &180.9 (\pm 6.8) &134.7 (\pm 6.8) &128.1 (\pm 6.9) &125.2 (\pm 6.7) &\tbcolorg 116.1 (\pm 6.6) \\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{Table}}}}}
&All Joints FDE &152.5 (\pm 1.1) &119.7 (\pm 0.9) &112.7 (\pm 0.8) &111.5 (\pm 0.8) &\tbcolorg 107.2 (\pm 0.8) \\
&Hands/Wrists FDE &195.4 (\pm 1.4) &153.8 (\pm 1.1) &146.0 (\pm 1.0) &144.3 (\pm 1.0) &\tbcolorg 138.9 (\pm 1.0) \\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{Avg.}}}}}
&All Joints FDE &124.2 (\pm 0.8) &94.9 (\pm 0.6) &87.6 (\pm 0.6) &87.3 (\pm 0.6) &\tbcolorg 82.2 (\pm 0.6) \\
&Hands/Wrists FDE &165.9 (\pm 1.1) &125.5 (\pm 0.8) &116.2 (\pm 0.8) &115.8 (\pm 0.7) &\tbcolorg 108.5 (\pm 0.7) \\
\bottomrule
\end{tabular}
}

\caption{Average forecast metrics (in mm) for all models across all CoMaD Human-Human datasets.}
\label{tab:forecasting_metrics}
\end{table*}



==> tables/table2.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{ccccccccccc}
\toprule
% & Models $\xrightarrow{}$  & \multicolumn{2}{c}{\textsc{Baselines}} && \multicolumn{6}{c}{\textsc{Learning-Based}}\\  \cmidrule{3-4} \cmidrule{6-11}
& Metrics (mm) $\downarrow$  & {\textsc{Only PreTrain}} & {\textsc{Only FineTuned}} & {\textsc{Marginal}} & {\textsc{InteRACT}} & {\textsc{InteRACT + Align}}\\   
% & & ADE & FDE && ADE & FDE  && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE\\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{Cab.}}}}}
&All Joints FDE &123.6 (\pm 2.4) &71.5 (\pm 1.7) &65.8 (\pm 1.6) &65.0 (\pm 1.6) &62.5 (\pm 1.5)\\
&Hands/Wrists FDE &155.3 (\pm 3.1) &87.4 (\pm 2.2) &79.4 (\pm 2.0) &77.8 (\pm 1.9) &75.2 (\pm 1.9)\\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}
{\textsc{\scriptsize{Table}}}}}
&All Joints FDE &82.9 (\pm 1.9) &47.9 (\pm 1.2) &45.2 (\pm 1.4) &42.9 (\pm 1.3) &42.5 (\pm 1.3)\\
&Hands/Wrists FDE &97.1 (\pm 2.1) &54.4 (\pm 1.4) &51.1 (\pm 1.6) &47.5 (\pm 1.4) &46.8 (\pm 1.4)\\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}
{\textsc{\scriptsize{Cart}}}}}
&All Joints FDE &97.1 (\pm 2.1) &58.3 (\pm 1.4) &50.2 (\pm 1.2) &49.8 (\pm 1.3) &49.3 (\pm 1.2)\\
&Hands/Wrists FDE &109.1 (\pm 2.2) &64.4 (\pm 1.6) &56.1 (\pm 1.4) &55.1 (\pm 1.4) &54.6 (\pm 1.4)\\
\midrule
\parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}
{\textsc{\scriptsize{Avg.}}}}}
&All Joints FDE &102.8 (\pm 1.3) &60.3 (\pm 0.9) &54.4 (\pm 0.8) &53.4 (\pm 0.8) &52.2 (\pm 0.8)\\
&Hands/Wrists FDE &122.3 (\pm 1.6) &69.9 (\pm 1.1) &63.0 (\pm 1.0) &61.1 (\pm 1.0) &59.9 (\pm 1.0)\\
\bottomrule
\end{tabular}
}

\caption{Average forecast metrics (in mm) for all models across all CoMaD Human-Robot datasets.}
\label{tab:forecasting_metrics_hr}
\end{table*}



==> tables/table3.tex <==
\begin{table}[t!]
\centering

\begin{tabular}{ccc}
\toprule
FDE (in mm) $\rightarrow$ & All Joints & Wrist and Hand \\
\midrule
% {\textsc{Marginal} - Only AMASS} & $417.2 (\pm 22.6)$ & $461.2 (\pm 22.3)$\\
{\textsc{Only FineTuned} & $424.9 (\pm 25.8)$& $446.3 (\pm 24.1)$\\
{\textsc{Marginal}} & $416.4 (\pm 24.1)$& $442.7 (\pm 23.0)$\\
\textsc{Marginal} (+ Hist) \cite{Wang2021MultiPerson3M} & $414.0 (\pm 23.9)$ & $444.7 (\pm 23.0)$\\
{\textsc{InteRACT} (ours)} & $\mathbf{412.6 (\pm 21.2)}$& $\mathbf{437.5 (\pm 20.0)}$\\
\bottomrule
\end{tabular}


\caption{Average prediction metrics (in mm) for all models on the CMU-MoCap dataset.}
\label{table:forecasting_metrics_cmu}
\end{table}

% \begin{table*}[t!]
% \centering
% \resizebox{\textwidth}{!}
% {
% \begin{tabular}{ccccccccccc}
% \toprule
% % & Models $\xrightarrow{}$  & \multicolumn{2}{c}{\textsc{Baselines}} && \multicolumn{6}{c}{\textsc{Learning-Based}}\\  \cmidrule{3-4} \cmidrule{6-11}
% & Metrics (mm) $\downarrow$  & {\textsc{Only PreTrain}} & {\textsc{Only FineTune}} & {\textsc{Marginal}} &{\textsc{Marginal-AllHist} \cite{Wang2021MultiPerson3M}} & {\textsc{InteRACT}}\\   
% % & & ADE & FDE && ADE & FDE  && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE\\
% \midrule
% \parbox[t]{2}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{\scriptsize{CMU}}}}}
% &All Joints FDE &417.2 (\pm 22.6) &424.9 (\pm 25.8) &416.4 (\pm 24.1) &445.9 (\pm 25.3) &\tbcolorg 412.6 (\pm 21.2) \\
% &Hands/Wrists FDE &461.2 (\pm 22.3) &446.3 (\pm 24.1) &442.7 (\pm 23.0) &472.8 (\pm 23.8) &\tbcolorg 437.5 (\pm 20.0) \\
% \bottomrule
% \end{tabular}
% }

% \caption{Average forecast metrics (in mm) for all models on the CMU-MoCap dataset.}
% \label{tab:forecasting_metrics_cmu}
% \end{table*}


